A homogenized constrained mixture model of cardiac growth and remodeling: Analyzing mechanobiological stability and reversal

Cardiac growth and remodeling (G&R) patterns change ventricular size, shape, and function both globally and locally. Biomechanical, neurohormonal, and genetic stimuli drive these patterns through changes in myocyte dimension and fibrosis. We propose a novel microstructure-motivated model that predicts organ-scale G&R in the heart based on the homogenized constrained mixture theory. Previous models, based on the kinematic growth theory, reproduced consequences of G&R in bulk myocardial tissue by prescribing the direction and extent of growth but neglected underlying cellular mechanisms. In our model, the direction and extent of G&R emerge naturally from intra- and extra cellular turnover processes in myocardial tissue constituents and their preferred homeostatic stretch state. We additionally propose a method to obtain a mechanobiologically equilibrated reference configuration. We test our model on an idealized 3D left ventricular geometry and demonstrate that our model aims to maintain tensional homeostasis in hypertension conditions. In a stability map, we identify regions of stable and unstable G&R from an identical parameter set with varying systolic pressures and growth factors. Furthermore, we show the extent of G&R reversal after returning the systolic pressure to baseline following stage 1 and 2 hypertension. A realistic model of organ-scale cardiac G&R has the potential to identify patients at risk of heart failure, enable personalized cardiac therapies, and facilitate the optimal design of medical devices.

==> figures/data/case140-1_gr_last.tex <==
\def\growthrangemin{0.974785695002}
\def\growthrangemax{1.10824013025}
\def\volumechangemin{0.0}
\def\volumechangemax{10.0}
\def\coordinaterangexmin{-0.299949278269}
\def\coordinaterangexmax{0.3}
\def\coordinaterangeymin{-0.549675929143}
\def\coordinaterangeymax{0.13}
\def\coordinaterangezmin{-0.3}
\def\coordinaterangezmax{0.3}
\def\meandispy{-0.042608840524}
\def\colormapmin{1.0}
\def\colormapmax{1.1}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(12,7,134)
        rgb255=(16,7,135)
        rgb255=(19,6,137)
        rgb255=(21,6,138)
        rgb255=(24,6,139)
        rgb255=(27,6,140)
        rgb255=(29,6,141)
        rgb255=(31,5,142)
        rgb255=(33,5,143)
        rgb255=(35,5,144)
        rgb255=(37,5,145)
        rgb255=(39,5,146)
        rgb255=(41,5,147)
        rgb255=(43,5,148)
        rgb255=(45,4,148)
        rgb255=(47,4,149)
        rgb255=(49,4,150)
        rgb255=(51,4,151)
        rgb255=(52,4,152)
        rgb255=(54,4,152)
        rgb255=(56,4,153)
        rgb255=(58,4,154)
        rgb255=(59,3,154)
        rgb255=(61,3,155)
        rgb255=(63,3,156)
        rgb255=(64,3,156)
        rgb255=(66,3,157)
        rgb255=(68,3,158)
        rgb255=(69,3,158)
        rgb255=(71,2,159)
        rgb255=(73,2,159)
        rgb255=(74,2,160)
        rgb255=(76,2,161)
        rgb255=(78,2,161)
        rgb255=(79,2,162)
        rgb255=(81,1,162)
        rgb255=(82,1,163)
        rgb255=(84,1,163)
        rgb255=(86,1,163)
        rgb255=(87,1,164)
        rgb255=(89,1,164)
        rgb255=(90,0,165)
        rgb255=(92,0,165)
        rgb255=(94,0,165)
        rgb255=(95,0,166)
        rgb255=(97,0,166)
        rgb255=(98,0,166)
        rgb255=(100,0,167)
        rgb255=(101,0,167)
        rgb255=(103,0,167)
        rgb255=(104,0,167)
        rgb255=(106,0,167)
        rgb255=(108,0,168)
        rgb255=(109,0,168)
        rgb255=(111,0,168)
        rgb255=(112,0,168)
        rgb255=(114,0,168)
        rgb255=(115,0,168)
        rgb255=(117,0,168)
        rgb255=(118,1,168)
        rgb255=(120,1,168)
        rgb255=(121,1,168)
        rgb255=(123,2,168)
        rgb255=(124,2,167)
        rgb255=(126,3,167)
        rgb255=(127,3,167)
        rgb255=(129,4,167)
        rgb255=(130,4,167)
        rgb255=(132,5,166)
        rgb255=(133,6,166)
        rgb255=(134,7,166)
        rgb255=(136,7,165)
        rgb255=(137,8,165)
        rgb255=(139,9,164)
        rgb255=(140,10,164)
        rgb255=(142,12,164)
        rgb255=(143,13,163)
        rgb255=(144,14,163)
        rgb255=(146,15,162)
        rgb255=(147,16,161)
        rgb255=(149,17,161)
        rgb255=(150,18,160)
        rgb255=(151,19,160)
        rgb255=(153,20,159)
        rgb255=(154,21,158)
        rgb255=(155,23,158)
        rgb255=(157,24,157)
        rgb255=(158,25,156)
        rgb255=(159,26,155)
        rgb255=(160,27,155)
        rgb255=(162,28,154)
        rgb255=(163,29,153)
        rgb255=(164,30,152)
        rgb255=(165,31,151)
        rgb255=(167,33,151)
        rgb255=(168,34,150)
        rgb255=(169,35,149)
        rgb255=(170,36,148)
        rgb255=(172,37,147)
        rgb255=(173,38,146)
        rgb255=(174,39,145)
        rgb255=(175,40,144)
        rgb255=(176,42,143)
        rgb255=(177,43,143)
        rgb255=(178,44,142)
        rgb255=(180,45,141)
        rgb255=(181,46,140)
        rgb255=(182,47,139)
        rgb255=(183,48,138)
        rgb255=(184,50,137)
        rgb255=(185,51,136)
        rgb255=(186,52,135)
        rgb255=(187,53,134)
        rgb255=(188,54,133)
        rgb255=(189,55,132)
        rgb255=(190,56,131)
        rgb255=(191,57,130)
        rgb255=(192,59,129)
        rgb255=(193,60,128)
        rgb255=(194,61,128)
        rgb255=(195,62,127)
        rgb255=(196,63,126)
        rgb255=(197,64,125)
        rgb255=(198,65,124)
        rgb255=(199,66,123)
        rgb255=(200,68,122)
        rgb255=(201,69,121)
        rgb255=(202,70,120)
        rgb255=(203,71,119)
        rgb255=(204,72,118)
        rgb255=(205,73,117)
        rgb255=(206,74,117)
        rgb255=(207,75,116)
        rgb255=(208,77,115)
        rgb255=(209,78,114)
        rgb255=(209,79,113)
        rgb255=(210,80,112)
        rgb255=(211,81,111)
        rgb255=(212,82,110)
        rgb255=(213,83,109)
        rgb255=(214,85,109)
        rgb255=(215,86,108)
        rgb255=(215,87,107)
        rgb255=(216,88,106)
        rgb255=(217,89,105)
        rgb255=(218,90,104)
        rgb255=(219,91,103)
        rgb255=(220,93,102)
        rgb255=(220,94,102)
        rgb255=(221,95,101)
        rgb255=(222,96,100)
        rgb255=(223,97,99)
        rgb255=(223,98,98)
        rgb255=(224,100,97)
        rgb255=(225,101,96)
        rgb255=(226,102,96)
        rgb255=(227,103,95)
        rgb255=(227,104,94)
        rgb255=(228,106,93)
        rgb255=(229,107,92)
        rgb255=(229,108,91)
        rgb255=(230,109,90)
        rgb255=(231,110,90)
        rgb255=(232,112,89)
        rgb255=(232,113,88)
        rgb255=(233,114,87)
        rgb255=(234,115,86)
        rgb255=(234,116,85)
        rgb255=(235,118,84)
        rgb255=(236,119,84)
        rgb255=(236,120,83)
        rgb255=(237,121,82)
        rgb255=(237,123,81)
        rgb255=(238,124,80)
        rgb255=(239,125,79)
        rgb255=(239,126,78)
        rgb255=(240,128,77)
        rgb255=(240,129,77)
        rgb255=(241,130,76)
        rgb255=(242,132,75)
        rgb255=(242,133,74)
        rgb255=(243,134,73)
        rgb255=(243,135,72)
        rgb255=(244,137,71)
        rgb255=(244,138,71)
        rgb255=(245,139,70)
        rgb255=(245,141,69)
        rgb255=(246,142,68)
        rgb255=(246,143,67)
        rgb255=(246,145,66)
        rgb255=(247,146,65)
        rgb255=(247,147,65)
        rgb255=(248,149,64)
        rgb255=(248,150,63)
        rgb255=(248,152,62)
        rgb255=(249,153,61)
        rgb255=(249,154,60)
        rgb255=(250,156,59)
        rgb255=(250,157,58)
        rgb255=(250,159,58)
        rgb255=(250,160,57)
        rgb255=(251,162,56)
        rgb255=(251,163,55)
        rgb255=(251,164,54)
        rgb255=(252,166,53)
        rgb255=(252,167,53)
        rgb255=(252,169,52)
        rgb255=(252,170,51)
        rgb255=(252,172,50)
        rgb255=(252,173,49)
        rgb255=(253,175,49)
        rgb255=(253,176,48)
        rgb255=(253,178,47)
        rgb255=(253,179,46)
        rgb255=(253,181,45)
        rgb255=(253,182,45)
        rgb255=(253,184,44)
        rgb255=(253,185,43)
        rgb255=(253,187,43)
        rgb255=(253,188,42)
        rgb255=(253,190,41)
        rgb255=(253,192,41)
        rgb255=(253,193,40)
        rgb255=(253,195,40)
        rgb255=(253,196,39)
        rgb255=(253,198,38)
        rgb255=(252,199,38)
        rgb255=(252,201,38)
        rgb255=(252,203,37)
        rgb255=(252,204,37)
        rgb255=(252,206,37)
        rgb255=(251,208,36)
        rgb255=(251,209,36)
        rgb255=(251,211,36)
        rgb255=(250,213,36)
        rgb255=(250,214,36)
        rgb255=(250,216,36)
        rgb255=(249,217,36)
        rgb255=(249,219,36)
        rgb255=(248,221,36)
        rgb255=(248,223,36)
        rgb255=(247,224,36)
        rgb255=(247,226,37)
        rgb255=(246,228,37)
        rgb255=(246,229,37)
        rgb255=(245,231,38)
        rgb255=(245,233,38)
        rgb255=(244,234,38)
        rgb255=(243,236,38)
        rgb255=(243,238,38)
        rgb255=(242,240,38)
        rgb255=(242,241,38)
        rgb255=(241,243,38)
        rgb255=(240,245,37)
        rgb255=(240,246,35)
        rgb255=(239,248,33)
    },
}
\def\thisimagewidth{871}
\def\thisimageheight{983}
\def\thisimagehalfwidth{435.5}
\def\thisimagehalfheight{491.5}


==> figures/data/case140-2_gr_last.tex <==
\def\growthrangemin{0.994132199835}
\def\growthrangemax{1.0181561853}
\def\volumechangemin{0.0}
\def\volumechangemax{10.0}
\def\coordinaterangexmin{-0.299949278269}
\def\coordinaterangexmax{0.3}
\def\coordinaterangeymin{-0.549675929143}
\def\coordinaterangeymax{0.13}
\def\coordinaterangezmin{-0.3}
\def\coordinaterangezmax{0.3}
\def\meandispy{0.00210358381054}
\def\colormapmin{1.0}
\def\colormapmax{1.1}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(12,7,134)
        rgb255=(16,7,135)
        rgb255=(19,6,137)
        rgb255=(21,6,138)
        rgb255=(24,6,139)
        rgb255=(27,6,140)
        rgb255=(29,6,141)
        rgb255=(31,5,142)
        rgb255=(33,5,143)
        rgb255=(35,5,144)
        rgb255=(37,5,145)
        rgb255=(39,5,146)
        rgb255=(41,5,147)
        rgb255=(43,5,148)
        rgb255=(45,4,148)
        rgb255=(47,4,149)
        rgb255=(49,4,150)
        rgb255=(51,4,151)
        rgb255=(52,4,152)
        rgb255=(54,4,152)
        rgb255=(56,4,153)
        rgb255=(58,4,154)
        rgb255=(59,3,154)
        rgb255=(61,3,155)
        rgb255=(63,3,156)
        rgb255=(64,3,156)
        rgb255=(66,3,157)
        rgb255=(68,3,158)
        rgb255=(69,3,158)
        rgb255=(71,2,159)
        rgb255=(73,2,159)
        rgb255=(74,2,160)
        rgb255=(76,2,161)
        rgb255=(78,2,161)
        rgb255=(79,2,162)
        rgb255=(81,1,162)
        rgb255=(82,1,163)
        rgb255=(84,1,163)
        rgb255=(86,1,163)
        rgb255=(87,1,164)
        rgb255=(89,1,164)
        rgb255=(90,0,165)
        rgb255=(92,0,165)
        rgb255=(94,0,165)
        rgb255=(95,0,166)
        rgb255=(97,0,166)
        rgb255=(98,0,166)
        rgb255=(100,0,167)
        rgb255=(101,0,167)
        rgb255=(103,0,167)
        rgb255=(104,0,167)
        rgb255=(106,0,167)
        rgb255=(108,0,168)
        rgb255=(109,0,168)
        rgb255=(111,0,168)
        rgb255=(112,0,168)
        rgb255=(114,0,168)
        rgb255=(115,0,168)
        rgb255=(117,0,168)
        rgb255=(118,1,168)
        rgb255=(120,1,168)
        rgb255=(121,1,168)
        rgb255=(123,2,168)
        rgb255=(124,2,167)
        rgb255=(126,3,167)
        rgb255=(127,3,167)
        rgb255=(129,4,167)
        rgb255=(130,4,167)
        rgb255=(132,5,166)
        rgb255=(133,6,166)
        rgb255=(134,7,166)
        rgb255=(136,7,165)
        rgb255=(137,8,165)
        rgb255=(139,9,164)
        rgb255=(140,10,164)
        rgb255=(142,12,164)
        rgb255=(143,13,163)
        rgb255=(144,14,163)
        rgb255=(146,15,162)
        rgb255=(147,16,161)
        rgb255=(149,17,161)
        rgb255=(150,18,160)
        rgb255=(151,19,160)
        rgb255=(153,20,159)
        rgb255=(154,21,158)
        rgb255=(155,23,158)
        rgb255=(157,24,157)
        rgb255=(158,25,156)
        rgb255=(159,26,155)
        rgb255=(160,27,155)
        rgb255=(162,28,154)
        rgb255=(163,29,153)
        rgb255=(164,30,152)
        rgb255=(165,31,151)
        rgb255=(167,33,151)
        rgb255=(168,34,150)
        rgb255=(169,35,149)
        rgb255=(170,36,148)
        rgb255=(172,37,147)
        rgb255=(173,38,146)
        rgb255=(174,39,145)
        rgb255=(175,40,144)
        rgb255=(176,42,143)
        rgb255=(177,43,143)
        rgb255=(178,44,142)
        rgb255=(180,45,141)
        rgb255=(181,46,140)
        rgb255=(182,47,139)
        rgb255=(183,48,138)
        rgb255=(184,50,137)
        rgb255=(185,51,136)
        rgb255=(186,52,135)
        rgb255=(187,53,134)
        rgb255=(188,54,133)
        rgb255=(189,55,132)
        rgb255=(190,56,131)
        rgb255=(191,57,130)
        rgb255=(192,59,129)
        rgb255=(193,60,128)
        rgb255=(194,61,128)
        rgb255=(195,62,127)
        rgb255=(196,63,126)
        rgb255=(197,64,125)
        rgb255=(198,65,124)
        rgb255=(199,66,123)
        rgb255=(200,68,122)
        rgb255=(201,69,121)
        rgb255=(202,70,120)
        rgb255=(203,71,119)
        rgb255=(204,72,118)
        rgb255=(205,73,117)
        rgb255=(206,74,117)
        rgb255=(207,75,116)
        rgb255=(208,77,115)
        rgb255=(209,78,114)
        rgb255=(209,79,113)
        rgb255=(210,80,112)
        rgb255=(211,81,111)
        rgb255=(212,82,110)
        rgb255=(213,83,109)
        rgb255=(214,85,109)
        rgb255=(215,86,108)
        rgb255=(215,87,107)
        rgb255=(216,88,106)
        rgb255=(217,89,105)
        rgb255=(218,90,104)
        rgb255=(219,91,103)
        rgb255=(220,93,102)
        rgb255=(220,94,102)
        rgb255=(221,95,101)
        rgb255=(222,96,100)
        rgb255=(223,97,99)
        rgb255=(223,98,98)
        rgb255=(224,100,97)
        rgb255=(225,101,96)
        rgb255=(226,102,96)
        rgb255=(227,103,95)
        rgb255=(227,104,94)
        rgb255=(228,106,93)
        rgb255=(229,107,92)
        rgb255=(229,108,91)
        rgb255=(230,109,90)
        rgb255=(231,110,90)
        rgb255=(232,112,89)
        rgb255=(232,113,88)
        rgb255=(233,114,87)
        rgb255=(234,115,86)
        rgb255=(234,116,85)
        rgb255=(235,118,84)
        rgb255=(236,119,84)
        rgb255=(236,120,83)
        rgb255=(237,121,82)
        rgb255=(237,123,81)
        rgb255=(238,124,80)
        rgb255=(239,125,79)
        rgb255=(239,126,78)
        rgb255=(240,128,77)
        rgb255=(240,129,77)
        rgb255=(241,130,76)
        rgb255=(242,132,75)
        rgb255=(242,133,74)
        rgb255=(243,134,73)
        rgb255=(243,135,72)
        rgb255=(244,137,71)
        rgb255=(244,138,71)
        rgb255=(245,139,70)
        rgb255=(245,141,69)
        rgb255=(246,142,68)
        rgb255=(246,143,67)
        rgb255=(246,145,66)
        rgb255=(247,146,65)
        rgb255=(247,147,65)
        rgb255=(248,149,64)
        rgb255=(248,150,63)
        rgb255=(248,152,62)
        rgb255=(249,153,61)
        rgb255=(249,154,60)
        rgb255=(250,156,59)
        rgb255=(250,157,58)
        rgb255=(250,159,58)
        rgb255=(250,160,57)
        rgb255=(251,162,56)
        rgb255=(251,163,55)
        rgb255=(251,164,54)
        rgb255=(252,166,53)
        rgb255=(252,167,53)
        rgb255=(252,169,52)
        rgb255=(252,170,51)
        rgb255=(252,172,50)
        rgb255=(252,173,49)
        rgb255=(253,175,49)
        rgb255=(253,176,48)
        rgb255=(253,178,47)
        rgb255=(253,179,46)
        rgb255=(253,181,45)
        rgb255=(253,182,45)
        rgb255=(253,184,44)
        rgb255=(253,185,43)
        rgb255=(253,187,43)
        rgb255=(253,188,42)
        rgb255=(253,190,41)
        rgb255=(253,192,41)
        rgb255=(253,193,40)
        rgb255=(253,195,40)
        rgb255=(253,196,39)
        rgb255=(253,198,38)
        rgb255=(252,199,38)
        rgb255=(252,201,38)
        rgb255=(252,203,37)
        rgb255=(252,204,37)
        rgb255=(252,206,37)
        rgb255=(251,208,36)
        rgb255=(251,209,36)
        rgb255=(251,211,36)
        rgb255=(250,213,36)
        rgb255=(250,214,36)
        rgb255=(250,216,36)
        rgb255=(249,217,36)
        rgb255=(249,219,36)
        rgb255=(248,221,36)
        rgb255=(248,223,36)
        rgb255=(247,224,36)
        rgb255=(247,226,37)
        rgb255=(246,228,37)
        rgb255=(246,229,37)
        rgb255=(245,231,38)
        rgb255=(245,233,38)
        rgb255=(244,234,38)
        rgb255=(243,236,38)
        rgb255=(243,238,38)
        rgb255=(242,240,38)
        rgb255=(242,241,38)
        rgb255=(241,243,38)
        rgb255=(240,245,37)
        rgb255=(240,246,35)
        rgb255=(239,248,33)
    },
}
\def\thisimagewidth{805}
\def\thisimageheight{933}
\def\thisimagehalfwidth{402.5}
\def\thisimagehalfheight{466.5}


==> figures/data/case180-1_gr_last.tex <==
\def\growthrangemin{0.919620898974632}
\def\growthrangemax{1.9170308555542361}
\def\volumechangemin{0.0}
\def\volumechangemax{90.99999999999999}
\def\coordinaterangexmin{-0.2999492782685655}
\def\coordinaterangexmax{0.3}
\def\coordinaterangeymin{-0.5496759291431355}
\def\coordinaterangeymax{0.13000000000000012}
\def\coordinaterangezmin{-0.3}
\def\coordinaterangezmax{0.3}
\def\meandispy{-0.22718412930243206}
\def\colormapmin{1.0}
\def\colormapmax{1.91}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(12,7,134)
        rgb255=(16,7,135)
        rgb255=(19,6,137)
        rgb255=(21,6,138)
        rgb255=(24,6,139)
        rgb255=(27,6,140)
        rgb255=(29,6,141)
        rgb255=(31,5,142)
        rgb255=(33,5,143)
        rgb255=(35,5,144)
        rgb255=(37,5,145)
        rgb255=(39,5,146)
        rgb255=(41,5,147)
        rgb255=(43,5,148)
        rgb255=(45,4,148)
        rgb255=(47,4,149)
        rgb255=(49,4,150)
        rgb255=(51,4,151)
        rgb255=(52,4,152)
        rgb255=(54,4,152)
        rgb255=(56,4,153)
        rgb255=(58,4,154)
        rgb255=(59,3,154)
        rgb255=(61,3,155)
        rgb255=(63,3,156)
        rgb255=(64,3,156)
        rgb255=(66,3,157)
        rgb255=(68,3,158)
        rgb255=(69,3,158)
        rgb255=(71,2,159)
        rgb255=(73,2,159)
        rgb255=(74,2,160)
        rgb255=(76,2,161)
        rgb255=(78,2,161)
        rgb255=(79,2,162)
        rgb255=(81,1,162)
        rgb255=(82,1,163)
        rgb255=(84,1,163)
        rgb255=(86,1,163)
        rgb255=(87,1,164)
        rgb255=(89,1,164)
        rgb255=(90,0,165)
        rgb255=(92,0,165)
        rgb255=(94,0,165)
        rgb255=(95,0,166)
        rgb255=(97,0,166)
        rgb255=(98,0,166)
        rgb255=(100,0,167)
        rgb255=(101,0,167)
        rgb255=(103,0,167)
        rgb255=(104,0,167)
        rgb255=(106,0,167)
        rgb255=(108,0,168)
        rgb255=(109,0,168)
        rgb255=(111,0,168)
        rgb255=(112,0,168)
        rgb255=(114,0,168)
        rgb255=(115,0,168)
        rgb255=(117,0,168)
        rgb255=(118,1,168)
        rgb255=(120,1,168)
        rgb255=(121,1,168)
        rgb255=(123,2,168)
        rgb255=(124,2,167)
        rgb255=(126,3,167)
        rgb255=(127,3,167)
        rgb255=(129,4,167)
        rgb255=(130,4,167)
        rgb255=(132,5,166)
        rgb255=(133,6,166)
        rgb255=(134,7,166)
        rgb255=(136,7,165)
        rgb255=(137,8,165)
        rgb255=(139,9,164)
        rgb255=(140,10,164)
        rgb255=(142,12,164)
        rgb255=(143,13,163)
        rgb255=(144,14,163)
        rgb255=(146,15,162)
        rgb255=(147,16,161)
        rgb255=(149,17,161)
        rgb255=(150,18,160)
        rgb255=(151,19,160)
        rgb255=(153,20,159)
        rgb255=(154,21,158)
        rgb255=(155,23,158)
        rgb255=(157,24,157)
        rgb255=(158,25,156)
        rgb255=(159,26,155)
        rgb255=(160,27,155)
        rgb255=(162,28,154)
        rgb255=(163,29,153)
        rgb255=(164,30,152)
        rgb255=(165,31,151)
        rgb255=(167,33,151)
        rgb255=(168,34,150)
        rgb255=(169,35,149)
        rgb255=(170,36,148)
        rgb255=(172,37,147)
        rgb255=(173,38,146)
        rgb255=(174,39,145)
        rgb255=(175,40,144)
        rgb255=(176,42,143)
        rgb255=(177,43,143)
        rgb255=(178,44,142)
        rgb255=(180,45,141)
        rgb255=(181,46,140)
        rgb255=(182,47,139)
        rgb255=(183,48,138)
        rgb255=(184,50,137)
        rgb255=(185,51,136)
        rgb255=(186,52,135)
        rgb255=(187,53,134)
        rgb255=(188,54,133)
        rgb255=(189,55,132)
        rgb255=(190,56,131)
        rgb255=(191,57,130)
        rgb255=(192,59,129)
        rgb255=(193,60,128)
        rgb255=(194,61,128)
        rgb255=(195,62,127)
        rgb255=(196,63,126)
        rgb255=(197,64,125)
        rgb255=(198,65,124)
        rgb255=(199,66,123)
        rgb255=(200,68,122)
        rgb255=(201,69,121)
        rgb255=(202,70,120)
        rgb255=(203,71,119)
        rgb255=(204,72,118)
        rgb255=(205,73,117)
        rgb255=(206,74,117)
        rgb255=(207,75,116)
        rgb255=(208,77,115)
        rgb255=(209,78,114)
        rgb255=(209,79,113)
        rgb255=(210,80,112)
        rgb255=(211,81,111)
        rgb255=(212,82,110)
        rgb255=(213,83,109)
        rgb255=(214,85,109)
        rgb255=(215,86,108)
        rgb255=(215,87,107)
        rgb255=(216,88,106)
        rgb255=(217,89,105)
        rgb255=(218,90,104)
        rgb255=(219,91,103)
        rgb255=(220,93,102)
        rgb255=(220,94,102)
        rgb255=(221,95,101)
        rgb255=(222,96,100)
        rgb255=(223,97,99)
        rgb255=(223,98,98)
        rgb255=(224,100,97)
        rgb255=(225,101,96)
        rgb255=(226,102,96)
        rgb255=(227,103,95)
        rgb255=(227,104,94)
        rgb255=(228,106,93)
        rgb255=(229,107,92)
        rgb255=(229,108,91)
        rgb255=(230,109,90)
        rgb255=(231,110,90)
        rgb255=(232,112,89)
        rgb255=(232,113,88)
        rgb255=(233,114,87)
        rgb255=(234,115,86)
        rgb255=(234,116,85)
        rgb255=(235,118,84)
        rgb255=(236,119,84)
        rgb255=(236,120,83)
        rgb255=(237,121,82)
        rgb255=(237,123,81)
        rgb255=(238,124,80)
        rgb255=(239,125,79)
        rgb255=(239,126,78)
        rgb255=(240,128,77)
        rgb255=(240,129,77)
        rgb255=(241,130,76)
        rgb255=(242,132,75)
        rgb255=(242,133,74)
        rgb255=(243,134,73)
        rgb255=(243,135,72)
        rgb255=(244,137,71)
        rgb255=(244,138,71)
        rgb255=(245,139,70)
        rgb255=(245,141,69)
        rgb255=(246,142,68)
        rgb255=(246,143,67)
        rgb255=(246,145,66)
        rgb255=(247,146,65)
        rgb255=(247,147,65)
        rgb255=(248,149,64)
        rgb255=(248,150,63)
        rgb255=(248,152,62)
        rgb255=(249,153,61)
        rgb255=(249,154,60)
        rgb255=(250,156,59)
        rgb255=(250,157,58)
        rgb255=(250,159,58)
        rgb255=(250,160,57)
        rgb255=(251,162,56)
        rgb255=(251,163,55)
        rgb255=(251,164,54)
        rgb255=(252,166,53)
        rgb255=(252,167,53)
        rgb255=(252,169,52)
        rgb255=(252,170,51)
        rgb255=(252,172,50)
        rgb255=(252,173,49)
        rgb255=(253,175,49)
        rgb255=(253,176,48)
        rgb255=(253,178,47)
        rgb255=(253,179,46)
        rgb255=(253,181,45)
        rgb255=(253,182,45)
        rgb255=(253,184,44)
        rgb255=(253,185,43)
        rgb255=(253,187,43)
        rgb255=(253,188,42)
        rgb255=(253,190,41)
        rgb255=(253,192,41)
        rgb255=(253,193,40)
        rgb255=(253,195,40)
        rgb255=(253,196,39)
        rgb255=(253,198,38)
        rgb255=(252,199,38)
        rgb255=(252,201,38)
        rgb255=(252,203,37)
        rgb255=(252,204,37)
        rgb255=(252,206,37)
        rgb255=(251,208,36)
        rgb255=(251,209,36)
        rgb255=(251,211,36)
        rgb255=(250,213,36)
        rgb255=(250,214,36)
        rgb255=(250,216,36)
        rgb255=(249,217,36)
        rgb255=(249,219,36)
        rgb255=(248,221,36)
        rgb255=(248,223,36)
        rgb255=(247,224,36)
        rgb255=(247,226,37)
        rgb255=(246,228,37)
        rgb255=(246,229,37)
        rgb255=(245,231,38)
        rgb255=(245,233,38)
        rgb255=(244,234,38)
        rgb255=(243,236,38)
        rgb255=(243,238,38)
        rgb255=(242,240,38)
        rgb255=(242,241,38)
        rgb255=(241,243,38)
        rgb255=(240,245,37)
        rgb255=(240,246,35)
        rgb255=(239,248,33)
    },
}
\def\thisimagewidth{1104}
\def\thisimageheight{1181}
\def\thisimagehalfwidth{552.0}
\def\thisimagehalfheight{590.5}

==> figures/data/case180b-1_gr_last.tex <==
\def\growthrangemin{0.95472275518}
\def\growthrangemax{1.26635514319}
\def\volumechangemin{0.0}
\def\volumechangemax{30.0}
\def\coordinaterangexmin{-0.299949278269}
\def\coordinaterangexmax{0.3}
\def\coordinaterangeymin{-0.549675929143}
\def\coordinaterangeymax{0.13}
\def\coordinaterangezmin{-0.3}
\def\coordinaterangezmax{0.3}
\def\meandispy{-0.0983137870907}
\def\colormapmin{1.0}
\def\colormapmax{1.3}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(12,7,134)
        rgb255=(16,7,135)
        rgb255=(19,6,137)
        rgb255=(21,6,138)
        rgb255=(24,6,139)
        rgb255=(27,6,140)
        rgb255=(29,6,141)
        rgb255=(31,5,142)
        rgb255=(33,5,143)
        rgb255=(35,5,144)
        rgb255=(37,5,145)
        rgb255=(39,5,146)
        rgb255=(41,5,147)
        rgb255=(43,5,148)
        rgb255=(45,4,148)
        rgb255=(47,4,149)
        rgb255=(49,4,150)
        rgb255=(51,4,151)
        rgb255=(52,4,152)
        rgb255=(54,4,152)
        rgb255=(56,4,153)
        rgb255=(58,4,154)
        rgb255=(59,3,154)
        rgb255=(61,3,155)
        rgb255=(63,3,156)
        rgb255=(64,3,156)
        rgb255=(66,3,157)
        rgb255=(68,3,158)
        rgb255=(69,3,158)
        rgb255=(71,2,159)
        rgb255=(73,2,159)
        rgb255=(74,2,160)
        rgb255=(76,2,161)
        rgb255=(78,2,161)
        rgb255=(79,2,162)
        rgb255=(81,1,162)
        rgb255=(82,1,163)
        rgb255=(84,1,163)
        rgb255=(86,1,163)
        rgb255=(87,1,164)
        rgb255=(89,1,164)
        rgb255=(90,0,165)
        rgb255=(92,0,165)
        rgb255=(94,0,165)
        rgb255=(95,0,166)
        rgb255=(97,0,166)
        rgb255=(98,0,166)
        rgb255=(100,0,167)
        rgb255=(101,0,167)
        rgb255=(103,0,167)
        rgb255=(104,0,167)
        rgb255=(106,0,167)
        rgb255=(108,0,168)
        rgb255=(109,0,168)
        rgb255=(111,0,168)
        rgb255=(112,0,168)
        rgb255=(114,0,168)
        rgb255=(115,0,168)
        rgb255=(117,0,168)
        rgb255=(118,1,168)
        rgb255=(120,1,168)
        rgb255=(121,1,168)
        rgb255=(123,2,168)
        rgb255=(124,2,167)
        rgb255=(126,3,167)
        rgb255=(127,3,167)
        rgb255=(129,4,167)
        rgb255=(130,4,167)
        rgb255=(132,5,166)
        rgb255=(133,6,166)
        rgb255=(134,7,166)
        rgb255=(136,7,165)
        rgb255=(137,8,165)
        rgb255=(139,9,164)
        rgb255=(140,10,164)
        rgb255=(142,12,164)
        rgb255=(143,13,163)
        rgb255=(144,14,163)
        rgb255=(146,15,162)
        rgb255=(147,16,161)
        rgb255=(149,17,161)
        rgb255=(150,18,160)
        rgb255=(151,19,160)
        rgb255=(153,20,159)
        rgb255=(154,21,158)
        rgb255=(155,23,158)
        rgb255=(157,24,157)
        rgb255=(158,25,156)
        rgb255=(159,26,155)
        rgb255=(160,27,155)
        rgb255=(162,28,154)
        rgb255=(163,29,153)
        rgb255=(164,30,152)
        rgb255=(165,31,151)
        rgb255=(167,33,151)
        rgb255=(168,34,150)
        rgb255=(169,35,149)
        rgb255=(170,36,148)
        rgb255=(172,37,147)
        rgb255=(173,38,146)
        rgb255=(174,39,145)
        rgb255=(175,40,144)
        rgb255=(176,42,143)
        rgb255=(177,43,143)
        rgb255=(178,44,142)
        rgb255=(180,45,141)
        rgb255=(181,46,140)
        rgb255=(182,47,139)
        rgb255=(183,48,138)
        rgb255=(184,50,137)
        rgb255=(185,51,136)
        rgb255=(186,52,135)
        rgb255=(187,53,134)
        rgb255=(188,54,133)
        rgb255=(189,55,132)
        rgb255=(190,56,131)
        rgb255=(191,57,130)
        rgb255=(192,59,129)
        rgb255=(193,60,128)
        rgb255=(194,61,128)
        rgb255=(195,62,127)
        rgb255=(196,63,126)
        rgb255=(197,64,125)
        rgb255=(198,65,124)
        rgb255=(199,66,123)
        rgb255=(200,68,122)
        rgb255=(201,69,121)
        rgb255=(202,70,120)
        rgb255=(203,71,119)
        rgb255=(204,72,118)
        rgb255=(205,73,117)
        rgb255=(206,74,117)
        rgb255=(207,75,116)
        rgb255=(208,77,115)
        rgb255=(209,78,114)
        rgb255=(209,79,113)
        rgb255=(210,80,112)
        rgb255=(211,81,111)
        rgb255=(212,82,110)
        rgb255=(213,83,109)
        rgb255=(214,85,109)
        rgb255=(215,86,108)
        rgb255=(215,87,107)
        rgb255=(216,88,106)
        rgb255=(217,89,105)
        rgb255=(218,90,104)
        rgb255=(219,91,103)
        rgb255=(220,93,102)
        rgb255=(220,94,102)
        rgb255=(221,95,101)
        rgb255=(222,96,100)
        rgb255=(223,97,99)
        rgb255=(223,98,98)
        rgb255=(224,100,97)
        rgb255=(225,101,96)
        rgb255=(226,102,96)
        rgb255=(227,103,95)
        rgb255=(227,104,94)
        rgb255=(228,106,93)
        rgb255=(229,107,92)
        rgb255=(229,108,91)
        rgb255=(230,109,90)
        rgb255=(231,110,90)
        rgb255=(232,112,89)
        rgb255=(232,113,88)
        rgb255=(233,114,87)
        rgb255=(234,115,86)
        rgb255=(234,116,85)
        rgb255=(235,118,84)
        rgb255=(236,119,84)
        rgb255=(236,120,83)
        rgb255=(237,121,82)
        rgb255=(237,123,81)
        rgb255=(238,124,80)
        rgb255=(239,125,79)
        rgb255=(239,126,78)
        rgb255=(240,128,77)
        rgb255=(240,129,77)
        rgb255=(241,130,76)
        rgb255=(242,132,75)
        rgb255=(242,133,74)
        rgb255=(243,134,73)
        rgb255=(243,135,72)
        rgb255=(244,137,71)
        rgb255=(244,138,71)
        rgb255=(245,139,70)
        rgb255=(245,141,69)
        rgb255=(246,142,68)
        rgb255=(246,143,67)
        rgb255=(246,145,66)
        rgb255=(247,146,65)
        rgb255=(247,147,65)
        rgb255=(248,149,64)
        rgb255=(248,150,63)
        rgb255=(248,152,62)
        rgb255=(249,153,61)
        rgb255=(249,154,60)
        rgb255=(250,156,59)
        rgb255=(250,157,58)
        rgb255=(250,159,58)
        rgb255=(250,160,57)
        rgb255=(251,162,56)
        rgb255=(251,163,55)
        rgb255=(251,164,54)
        rgb255=(252,166,53)
        rgb255=(252,167,53)
        rgb255=(252,169,52)
        rgb255=(252,170,51)
        rgb255=(252,172,50)
        rgb255=(252,173,49)
        rgb255=(253,175,49)
        rgb255=(253,176,48)
        rgb255=(253,178,47)
        rgb255=(253,179,46)
        rgb255=(253,181,45)
        rgb255=(253,182,45)
        rgb255=(253,184,44)
        rgb255=(253,185,43)
        rgb255=(253,187,43)
        rgb255=(253,188,42)
        rgb255=(253,190,41)
        rgb255=(253,192,41)
        rgb255=(253,193,40)
        rgb255=(253,195,40)
        rgb255=(253,196,39)
        rgb255=(253,198,38)
        rgb255=(252,199,38)
        rgb255=(252,201,38)
        rgb255=(252,203,37)
        rgb255=(252,204,37)
        rgb255=(252,206,37)
        rgb255=(251,208,36)
        rgb255=(251,209,36)
        rgb255=(251,211,36)
        rgb255=(250,213,36)
        rgb255=(250,214,36)
        rgb255=(250,216,36)
        rgb255=(249,217,36)
        rgb255=(249,219,36)
        rgb255=(248,221,36)
        rgb255=(248,223,36)
        rgb255=(247,224,36)
        rgb255=(247,226,37)
        rgb255=(246,228,37)
        rgb255=(246,229,37)
        rgb255=(245,231,38)
        rgb255=(245,233,38)
        rgb255=(244,234,38)
        rgb255=(243,236,38)
        rgb255=(243,238,38)
        rgb255=(242,240,38)
        rgb255=(242,241,38)
        rgb255=(241,243,38)
        rgb255=(240,245,37)
        rgb255=(240,246,35)
        rgb255=(239,248,33)
    },
}
\def\thisimagewidth{924}
\def\thisimageheight{1021}
\def\thisimagehalfwidth{462.0}
\def\thisimagehalfheight{510.5}


==> figures/data/case180b-3_gr_last.tex <==
\def\growthrangemin{0.984147455276}
\def\growthrangemax{1.10332979312}
\def\volumechangemin{0.0}
\def\volumechangemax{30.0}
\def\coordinaterangexmin{-0.299949278269}
\def\coordinaterangexmax{0.3}
\def\coordinaterangeymin{-0.549675929143}
\def\coordinaterangeymax{0.13}
\def\coordinaterangezmin{-0.3}
\def\coordinaterangezmax{0.3}
\def\meandispy{0.00952178233966}
\def\colormapmin{1.0}
\def\colormapmax{1.3}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(12,7,134)
        rgb255=(16,7,135)
        rgb255=(19,6,137)
        rgb255=(21,6,138)
        rgb255=(24,6,139)
        rgb255=(27,6,140)
        rgb255=(29,6,141)
        rgb255=(31,5,142)
        rgb255=(33,5,143)
        rgb255=(35,5,144)
        rgb255=(37,5,145)
        rgb255=(39,5,146)
        rgb255=(41,5,147)
        rgb255=(43,5,148)
        rgb255=(45,4,148)
        rgb255=(47,4,149)
        rgb255=(49,4,150)
        rgb255=(51,4,151)
        rgb255=(52,4,152)
        rgb255=(54,4,152)
        rgb255=(56,4,153)
        rgb255=(58,4,154)
        rgb255=(59,3,154)
        rgb255=(61,3,155)
        rgb255=(63,3,156)
        rgb255=(64,3,156)
        rgb255=(66,3,157)
        rgb255=(68,3,158)
        rgb255=(69,3,158)
        rgb255=(71,2,159)
        rgb255=(73,2,159)
        rgb255=(74,2,160)
        rgb255=(76,2,161)
        rgb255=(78,2,161)
        rgb255=(79,2,162)
        rgb255=(81,1,162)
        rgb255=(82,1,163)
        rgb255=(84,1,163)
        rgb255=(86,1,163)
        rgb255=(87,1,164)
        rgb255=(89,1,164)
        rgb255=(90,0,165)
        rgb255=(92,0,165)
        rgb255=(94,0,165)
        rgb255=(95,0,166)
        rgb255=(97,0,166)
        rgb255=(98,0,166)
        rgb255=(100,0,167)
        rgb255=(101,0,167)
        rgb255=(103,0,167)
        rgb255=(104,0,167)
        rgb255=(106,0,167)
        rgb255=(108,0,168)
        rgb255=(109,0,168)
        rgb255=(111,0,168)
        rgb255=(112,0,168)
        rgb255=(114,0,168)
        rgb255=(115,0,168)
        rgb255=(117,0,168)
        rgb255=(118,1,168)
        rgb255=(120,1,168)
        rgb255=(121,1,168)
        rgb255=(123,2,168)
        rgb255=(124,2,167)
        rgb255=(126,3,167)
        rgb255=(127,3,167)
        rgb255=(129,4,167)
        rgb255=(130,4,167)
        rgb255=(132,5,166)
        rgb255=(133,6,166)
        rgb255=(134,7,166)
        rgb255=(136,7,165)
        rgb255=(137,8,165)
        rgb255=(139,9,164)
        rgb255=(140,10,164)
        rgb255=(142,12,164)
        rgb255=(143,13,163)
        rgb255=(144,14,163)
        rgb255=(146,15,162)
        rgb255=(147,16,161)
        rgb255=(149,17,161)
        rgb255=(150,18,160)
        rgb255=(151,19,160)
        rgb255=(153,20,159)
        rgb255=(154,21,158)
        rgb255=(155,23,158)
        rgb255=(157,24,157)
        rgb255=(158,25,156)
        rgb255=(159,26,155)
        rgb255=(160,27,155)
        rgb255=(162,28,154)
        rgb255=(163,29,153)
        rgb255=(164,30,152)
        rgb255=(165,31,151)
        rgb255=(167,33,151)
        rgb255=(168,34,150)
        rgb255=(169,35,149)
        rgb255=(170,36,148)
        rgb255=(172,37,147)
        rgb255=(173,38,146)
        rgb255=(174,39,145)
        rgb255=(175,40,144)
        rgb255=(176,42,143)
        rgb255=(177,43,143)
        rgb255=(178,44,142)
        rgb255=(180,45,141)
        rgb255=(181,46,140)
        rgb255=(182,47,139)
        rgb255=(183,48,138)
        rgb255=(184,50,137)
        rgb255=(185,51,136)
        rgb255=(186,52,135)
        rgb255=(187,53,134)
        rgb255=(188,54,133)
        rgb255=(189,55,132)
        rgb255=(190,56,131)
        rgb255=(191,57,130)
        rgb255=(192,59,129)
        rgb255=(193,60,128)
        rgb255=(194,61,128)
        rgb255=(195,62,127)
        rgb255=(196,63,126)
        rgb255=(197,64,125)
        rgb255=(198,65,124)
        rgb255=(199,66,123)
        rgb255=(200,68,122)
        rgb255=(201,69,121)
        rgb255=(202,70,120)
        rgb255=(203,71,119)
        rgb255=(204,72,118)
        rgb255=(205,73,117)
        rgb255=(206,74,117)
        rgb255=(207,75,116)
        rgb255=(208,77,115)
        rgb255=(209,78,114)
        rgb255=(209,79,113)
        rgb255=(210,80,112)
        rgb255=(211,81,111)
        rgb255=(212,82,110)
        rgb255=(213,83,109)
        rgb255=(214,85,109)
        rgb255=(215,86,108)
        rgb255=(215,87,107)
        rgb255=(216,88,106)
        rgb255=(217,89,105)
        rgb255=(218,90,104)
        rgb255=(219,91,103)
        rgb255=(220,93,102)
        rgb255=(220,94,102)
        rgb255=(221,95,101)
        rgb255=(222,96,100)
        rgb255=(223,97,99)
        rgb255=(223,98,98)
        rgb255=(224,100,97)
        rgb255=(225,101,96)
        rgb255=(226,102,96)
        rgb255=(227,103,95)
        rgb255=(227,104,94)
        rgb255=(228,106,93)
        rgb255=(229,107,92)
        rgb255=(229,108,91)
        rgb255=(230,109,90)
        rgb255=(231,110,90)
        rgb255=(232,112,89)
        rgb255=(232,113,88)
        rgb255=(233,114,87)
        rgb255=(234,115,86)
        rgb255=(234,116,85)
        rgb255=(235,118,84)
        rgb255=(236,119,84)
        rgb255=(236,120,83)
        rgb255=(237,121,82)
        rgb255=(237,123,81)
        rgb255=(238,124,80)
        rgb255=(239,125,79)
        rgb255=(239,126,78)
        rgb255=(240,128,77)
        rgb255=(240,129,77)
        rgb255=(241,130,76)
        rgb255=(242,132,75)
        rgb255=(242,133,74)
        rgb255=(243,134,73)
        rgb255=(243,135,72)
        rgb255=(244,137,71)
        rgb255=(244,138,71)
        rgb255=(245,139,70)
        rgb255=(245,141,69)
        rgb255=(246,142,68)
        rgb255=(246,143,67)
        rgb255=(246,145,66)
        rgb255=(247,146,65)
        rgb255=(247,147,65)
        rgb255=(248,149,64)
        rgb255=(248,150,63)
        rgb255=(248,152,62)
        rgb255=(249,153,61)
        rgb255=(249,154,60)
        rgb255=(250,156,59)
        rgb255=(250,157,58)
        rgb255=(250,159,58)
        rgb255=(250,160,57)
        rgb255=(251,162,56)
        rgb255=(251,163,55)
        rgb255=(251,164,54)
        rgb255=(252,166,53)
        rgb255=(252,167,53)
        rgb255=(252,169,52)
        rgb255=(252,170,51)
        rgb255=(252,172,50)
        rgb255=(252,173,49)
        rgb255=(253,175,49)
        rgb255=(253,176,48)
        rgb255=(253,178,47)
        rgb255=(253,179,46)
        rgb255=(253,181,45)
        rgb255=(253,182,45)
        rgb255=(253,184,44)
        rgb255=(253,185,43)
        rgb255=(253,187,43)
        rgb255=(253,188,42)
        rgb255=(253,190,41)
        rgb255=(253,192,41)
        rgb255=(253,193,40)
        rgb255=(253,195,40)
        rgb255=(253,196,39)
        rgb255=(253,198,38)
        rgb255=(252,199,38)
        rgb255=(252,201,38)
        rgb255=(252,203,37)
        rgb255=(252,204,37)
        rgb255=(252,206,37)
        rgb255=(251,208,36)
        rgb255=(251,209,36)
        rgb255=(251,211,36)
        rgb255=(250,213,36)
        rgb255=(250,214,36)
        rgb255=(250,216,36)
        rgb255=(249,217,36)
        rgb255=(249,219,36)
        rgb255=(248,221,36)
        rgb255=(248,223,36)
        rgb255=(247,224,36)
        rgb255=(247,226,37)
        rgb255=(246,228,37)
        rgb255=(246,229,37)
        rgb255=(245,231,38)
        rgb255=(245,233,38)
        rgb255=(244,234,38)
        rgb255=(243,236,38)
        rgb255=(243,238,38)
        rgb255=(242,240,38)
        rgb255=(242,241,38)
        rgb255=(241,243,38)
        rgb255=(240,245,37)
        rgb255=(240,246,35)
        rgb255=(239,248,33)
    },
}
\def\thisimagewidth{799}
\def\thisimageheight{930}
\def\thisimagehalfwidth{399.5}
\def\thisimagehalfheight{465.0}


==> figures/data/metrics_i180.tex <==
\def\myocytehomeostaticstressistagetwo{22.02277748047476}
\def\midcavityrefwallthicknessistagetwo{10.761044144526878}
\def\cavitydiameteristagetwo{37.992774309903595}
\def\timepointaistagetwo{0.0}
\def\pressureaistagetwo{120.0}
\def\myocytestressaistagetwo{22.022572791705613}
\def\diameteraistagetwo{37.96994287218595}
\def\wallthicknessaistagetwo{10.760549874663688}
\def\collagenmassfractionaistagetwo{0.10000215156363837}
\def\timepointbistagetwo{431.0}
\def\pressurebistagetwo{180.0}
\def\myocytestressbistagetwo{23.081851201642618}
\def\diameterbistagetwo{68.15562534064199}
\def\wallthicknessbistagetwo{7.446926607076746}
\def\collagenmassfractionbistagetwo{0.2538358330888966}


==> figures/data/metrics_r140.tex <==
\def\myocytehomeostaticstressrstageone{22.02277748047476}
\def\midcavityrefwallthicknessrstageone{10.761044144526878}
\def\cavitydiameterrstageone{37.992774309903595}
\def\timepointarstageone{0.0}
\def\pressurearstageone{120.0}
\def\myocytestressarstageone{22.022572791705613}
\def\diameterarstageone{37.96994287218595}
\def\wallthicknessarstageone{10.760549874663688}
\def\collagenmassfractionarstageone{0.10000215156363837}
\def\timepointbrstageone{1327.5}
\def\pressurebrstageone{140.0}
\def\myocytestressbrstageone{22.024184306673018}
\def\diameterbrstageone{45.51353178340367}
\def\wallthicknessbrstageone{9.501610117572215}
\def\collagenmassfractionbrstageone{0.12326430486261057}
\def\timepointcrstageone{1986.5}
\def\pressurecrstageone{120.0}
\def\myocytestresscrstageone{22.02170942201418}
\def\diametercrstageone{37.361336289673105}
\def\wallthicknesscrstageone{10.976419494614436}
\def\collagenmassfractioncrstageone{0.1028489457784486}


==> figures/data/metrics_r180.tex <==
\def\myocytehomeostaticstressrstagetwo{22.02277748047476}
\def\midcavityrefwallthicknessrstagetwo{10.761044144526878}
\def\cavitydiameterrstagetwo{37.992774309903595}
\def\timepointarstagetwo{0.0}
\def\pressurearstagetwo{120.0}
\def\myocytestressarstagetwo{22.022572791705613}
\def\diameterarstagetwo{37.96994287218595}
\def\wallthicknessarstagetwo{10.760549874663688}
\def\collagenmassfractionarstagetwo{0.10000215156363837}
\def\timepointbrstagetwo{151.0}
\def\pressurebrstagetwo{180.0}
\def\myocytestressbrstagetwo{23.093500400201027}
\def\diameterbrstagetwo{50.51660108418565}
\def\wallthicknessbrstagetwo{9.034558864255985}
\def\collagenmassfractionbrstagetwo{0.15300607334434727}
\def\timepointcrstagetwo{854.5}
\def\pressurecrstagetwo{120.0}
\def\myocytestresscrstagetwo{22.021677759616935}
\def\diametercrstagetwo{34.77923226886743}
\def\wallthicknesscrstagetwo{11.843814513633955}
\def\collagenmassfractioncrstagetwo{0.11438205128862164}


==> figures/data/pr_eigenvalue1.tex <==
\def\eigenvaluerangemin{0.5}
\def\eigenvaluerangemax{1.5}
\def\colormapmin{0.5}
\def\colormapmax{1.5}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(22,1,76)
        rgb255=(28,5,114)
        rgb255=(26,13,130)
        rgb255=(10,10,142)
        rgb255=(7,24,153)
        rgb255=(11,42,163)
        rgb255=(14,61,172)
        rgb255=(14,80,181)
        rgb255=(13,100,188)
        rgb255=(10,119,195)
        rgb255=(7,137,200)
        rgb255=(7,156,207)
        rgb255=(5,181,212)
        rgb255=(13,204,216)
        rgb255=(17,218,221)
        rgb255=(66,230,219)
        rgb255=(107,239,223)
        rgb255=(145,246,212)
        rgb255=(168,249,214)
        rgb255=(195,249,221)
        rgb255=(211,249,226)
        rgb255=(232,251,239)
        rgb255=(255,255,247)
        rgb255=(251,249,221)
        rgb255=(252,247,205)
        rgb255=(253,246,181)
        rgb255=(251,244,163)
        rgb255=(249,233,130)
        rgb255=(246,223,103)
        rgb255=(242,209,82)
        rgb255=(237,198,70)
        rgb255=(232,182,59)
        rgb255=(226,168,49)
        rgb255=(223,158,42)
        rgb255=(221,140,40)
        rgb255=(216,121,36)
        rgb255=(212,105,33)
        rgb255=(207,87,28)
        rgb255=(200,68,23)
        rgb255=(188,47,18)
        rgb255=(175,31,16)
        rgb255=(158,16,11)
        rgb255=(140,7,17)
        rgb255=(119,4,23)
        rgb255=(102,1,26)
        rgb255=(47,0,17)
    },
}
\def\thisimagewidth{1381}
\def\thisimageheight{1479}
\def\thisimagehalfwidth{690.5}
\def\thisimagehalfheight{739.5}


==> figures/data/pr_eigenvalue3.tex <==
\def\eigenvaluerangemin{0.5}
\def\eigenvaluerangemax{1.5}
\def\colormapmin{0.5}
\def\colormapmax{1.5}
\pgfplotsset{
    colormap={thisplotcolormap}{
        rgb255=(22,1,76)
        rgb255=(28,5,114)
        rgb255=(26,13,130)
        rgb255=(10,10,142)
        rgb255=(7,24,153)
        rgb255=(11,42,163)
        rgb255=(14,61,172)
        rgb255=(14,80,181)
        rgb255=(13,100,188)
        rgb255=(10,119,195)
        rgb255=(7,137,200)
        rgb255=(7,156,207)
        rgb255=(5,181,212)
        rgb255=(13,204,216)
        rgb255=(17,218,221)
        rgb255=(66,230,219)
        rgb255=(107,239,223)
        rgb255=(145,246,212)
        rgb255=(168,249,214)
        rgb255=(195,249,221)
        rgb255=(211,249,226)
        rgb255=(232,251,239)
        rgb255=(255,255,247)
        rgb255=(251,249,221)
        rgb255=(252,247,205)
        rgb255=(253,246,181)
        rgb255=(251,244,163)
        rgb255=(249,233,130)
        rgb255=(246,223,103)
        rgb255=(242,209,82)
        rgb255=(237,198,70)
        rgb255=(232,182,59)
        rgb255=(226,168,49)
        rgb255=(223,158,42)
        rgb255=(221,140,40)
        rgb255=(216,121,36)
        rgb255=(212,105,33)
        rgb255=(207,87,28)
        rgb255=(200,68,23)
        rgb255=(188,47,18)
        rgb255=(175,31,16)
        rgb255=(158,16,11)
        rgb255=(140,7,17)
        rgb255=(119,4,23)
        rgb255=(102,1,26)
        rgb255=(47,0,17)
    },
}
\def\thisimagewidth{1385}
\def\thisimageheight{1482}
\def\thisimagehalfwidth{692.5}
\def\thisimagehalfheight{741.0}


==> figures/pgfdefinitions.tex <==
\newcommand*{\plotwithstddev}[3][1]{   
    \addplot[name path=A,color=#2!70, forget plot] table [x=time, y expr={(\thisrow{average}+\thisrow{stddev})*#1}, col sep=comma]
        {#3};
    \addplot[name path=B,color=#2!70, forget plot] table [x=time, y expr={(\thisrow{average}-\thisrow{stddev})*#1}, col sep=comma]
        {#3};
    \addplot[#2!50,fill opacity=0.5, forget plot] fill between[of=A and B];

    \addplot[mark=none, line width=1pt, color=#2]
        table [x=time, y expr={(\thisrow{average})*#1}, col sep=comma]
            {#3};
}
\newcommand*{\timeplot}[3][average]{
    \addplot[mark=none, line width=1pt, color=#2 ]
    table [x=time, y=#1, col sep=comma]
        {#3};
}

==> supplementary_materials/figures/data/metrics_i180.tex <==
\def\myocytehomeostaticstressistagetwo{22.02277748047476}
\def\collagenahomeostaticstressistagetwo{5.16340598316476}
\def\collagenbhomeostaticstressistagetwo{5.16340598316476}
\def\collagenchomeostaticstressistagetwo{5.16340598316476}
\def\collagendhomeostaticstressistagetwo{5.16340598316476}
\def\midcavityrefwallthicknessistagetwo{10.761044144526878}
\def\cavitydiameteristagetwo{37.97108789828769}
\def\timepointaistagetwo{0.0}
\def\pressureaistagetwo{120.0}
\def\myocytestressaistagetwo{22.02257643915123}
\def\diameteraistagetwo{37.982982157439146}
\def\wallthicknessaistagetwo{10.760539770234908}
\def\collagenmassfractionaistagetwo{0.1000022361719026}
\def\collagenastressaistagetwo{5.162990524973489}
\def\collagenbstressaistagetwo{5.164316497551072}
\def\collagencstressaistagetwo{5.162804063777092}
\def\collagendstressaistagetwo{5.164507469317477}
\def\fiberamassfractionaistagetwo{0.5999973077248604}
\def\fiberbmassfractionaistagetwo{0.024999254137254324}
\def\fibercmassfractionaistagetwo{0.025001860320391627}
\def\fiberdmassfractionaistagetwo{0.024998324489738658}
\def\fiberemassfractionaistagetwo{0.025002797224517988}
\def\timepointbistagetwo{431.0}
\def\pressurebistagetwo{180.0}
\def\myocytestressbistagetwo{23.080600460769777}
\def\diameterbistagetwo{68.174556106555}
\def\wallthicknessbistagetwo{7.446502891513393}
\def\collagenmassfractionbistagetwo{0.2540101805038529}
\def\collagenastressbistagetwo{7.278541181835632}
\def\collagenbstressbistagetwo{7.203626378671096}
\def\collagencstressbistagetwo{7.167847984828654}
\def\collagendstressbistagetwo{7.310061859033193}
\def\fiberamassfractionbistagetwo{0.5339052558482369}
\def\fiberbmassfractionbistagetwo{0.06532460584412825}
\def\fibercmassfractionbistagetwo{0.06035347569072301}
\def\fiberdmassfractionbistagetwo{0.056423968828921554}
\def\fiberemassfractionbistagetwo{0.0719081301400801}


==> supplementary_materials/figures/data/metrics_r140.tex <==
\def\myocytehomeostaticstressrstageone{22.02277748047476}
\def\collagenahomeostaticstressrstageone{5.16340598316476}
\def\collagenbhomeostaticstressrstageone{5.16340598316476}
\def\collagenchomeostaticstressrstageone{5.16340598316476}
\def\collagendhomeostaticstressrstageone{5.16340598316476}
\def\midcavityrefwallthicknessrstageone{10.761044144526878}
\def\cavitydiameterrstageone{37.97108789828769}
\def\timepointarstageone{0.0}
\def\pressurearstageone{120.0}
\def\myocytestressarstageone{22.02257643915123}
\def\diameterarstageone{37.982982157439146}
\def\wallthicknessarstageone{10.760539770234908}
\def\collagenmassfractionarstageone{0.1000022361719026}
\def\collagenastressarstageone{5.162990524973489}
\def\collagenbstressarstageone{5.164316497551072}
\def\collagencstressarstageone{5.162804063777092}
\def\collagendstressarstageone{5.164507469317477}
\def\fiberamassfractionarstageone{0.5999973077248604}
\def\fiberbmassfractionarstageone{0.024999254137254324}
\def\fibercmassfractionarstageone{0.025001860320391627}
\def\fiberdmassfractionarstageone{0.024998324489738658}
\def\fiberemassfractionarstageone{0.025002797224517988}
\def\timepointbrstageone{1328.5}
\def\pressurebrstageone{140.0}
\def\myocytestressbrstageone{22.024182482227417}
\def\diameterbrstageone{45.487213640189964}
\def\wallthicknessbrstageone{9.501734110846582}
\def\collagenmassfractionbrstageone{0.12326161508607952}
\def\collagenastressbrstageone{5.166276401643611}
\def\collagenbstressbrstageone{5.165993458487153}
\def\collagencstressbrstageone{5.165958175847066}
\def\collagendstressbrstageone{5.166303868264748}
\def\fiberamassfractionbrstageone{0.5941728669965559}
\def\fiberbmassfractionbrstageone{0.031308684881475125}
\def\fibercmassfractionbrstageone{0.030290249030723092}
\def\fiberdmassfractionbrstageone{0.030121597922759296}
\def\fiberemassfractionbrstageone{0.031541083251122}
\def\timepointcrstageone{1988.5}
\def\pressurecrstageone{120.0}
\def\myocytestresscrstageone{22.02170744001227}
\def\diametercrstageone{37.355680653048026}
\def\wallthicknesscrstageone{10.976109457287103}
\def\collagenmassfractioncrstageone{0.1028483246693137}
\def\collagenastresscrstageone{5.161129162753281}
\def\collagenbstresscrstageone{5.161438415975875}
\def\collagencstresscrstageone{5.161464013749548}
\def\collagendstresscrstageone{5.161102754354906}
\def\fiberamassfractioncrstageone{0.5996067205775041}
\def\fiberbmassfractioncrstageone{0.02577041714223378}
\def\fibercmassfractioncrstageone{0.02563129141657564}
\def\fiberdmassfractioncrstageone{0.025532061348326016}
\def\fiberemassfractioncrstageone{0.025914554762178268}


==> supplementary_materials/figures/data/metrics_r180.tex <==
\def\myocytehomeostaticstressrstagetwo{22.02277748047476}
\def\collagenahomeostaticstressrstagetwo{5.16340598316476}
\def\collagenbhomeostaticstressrstagetwo{5.16340598316476}
\def\collagenchomeostaticstressrstagetwo{5.16340598316476}
\def\collagendhomeostaticstressrstagetwo{5.16340598316476}
\def\midcavityrefwallthicknessrstagetwo{10.761044144526878}
\def\cavitydiameterrstagetwo{37.97108789828769}
\def\timepointarstagetwo{0.0}
\def\pressurearstagetwo{120.0}
\def\myocytestressarstagetwo{22.02257643915123}
\def\diameterarstagetwo{37.982982157439146}
\def\wallthicknessarstagetwo{10.760539770234908}
\def\collagenmassfractionarstagetwo{0.1000022361719026}
\def\collagenastressarstagetwo{5.162990524973489}
\def\collagenbstressarstagetwo{5.164316497551072}
\def\collagencstressarstagetwo{5.162804063777092}
\def\collagendstressarstagetwo{5.164507469317477}
\def\fiberamassfractionarstagetwo{0.5999973077248604}
\def\fiberbmassfractionarstagetwo{0.024999254137254324}
\def\fibercmassfractionarstagetwo{0.025001860320391627}
\def\fiberdmassfractionarstagetwo{0.024998324489738658}
\def\fiberemassfractionarstagetwo{0.025002797224517988}
\def\timepointbrstagetwo{151.0}
\def\pressurebrstagetwo{180.0}
\def\myocytestressbrstagetwo{23.0919600700889}
\def\diameterbrstagetwo{50.564250217116616}
\def\wallthicknessbrstagetwo{9.031813817649843}
\def\collagenmassfractionbrstagetwo{0.1531581988486206}
\def\collagenastressbrstagetwo{7.345675502578698}
\def\collagenbstressbrstagetwo{7.165914081843303}
\def\collagencstressbrstagetwo{7.114711740364642}
\def\collagendstressbrstagetwo{7.395628650506253}
\def\fiberamassfractionbrstagetwo{0.5841669308433336}
\def\fiberbmassfractionbrstagetwo{0.038975737763679484}
\def\fibercmassfractionbrstagetwo{0.037076881815703816}
\def\fiberdmassfractionbrstagetwo{0.03576169288862181}
\def\fiberemassfractionbrstagetwo{0.041343886380615535}
\def\timepointcrstagetwo{855.5}
\def\pressurecrstagetwo{120.0}
\def\myocytestresscrstagetwo{22.021674414018996}
\def\diametercrstagetwo{34.746034631548746}
\def\wallthicknesscrstagetwo{11.842800468885063}
\def\collagenmassfractioncrstagetwo{0.11438786875882459}
\def\collagenastresscrstagetwo{5.161056260866821}
\def\collagenbstresscrstagetwo{5.161392309106018}
\def\collagencstresscrstagetwo{5.161426832189495}
\def\collagendstresscrstagetwo{5.161013152998169}
\def\fiberamassfractioncrstagetwo{0.5976683104361796}
\def\fiberbmassfractioncrstagetwo{0.028635070977934204}
\def\fibercmassfractioncrstagetwo{0.028285862128191445}
\def\fiberdmassfractioncrstagetwo{0.027519644196721368}
\def\fiberemassfractioncrstagetwo{0.02994729145597757}


==> supplementary_materials/figures/data/metrics_s140_0.33.tex <==
\def\myocytehomeostaticstresspstagetwoa{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoa{10.761044144526878}
\def\cavitydiameterpstagetwoa{37.97807748655915}
\def\timepointapstagetwoa{0.0}
\def\pressureapstagetwoa{120.0}
\def\myocytestressapstagetwoa{22.021899769774404}
\def\diameterapstagetwoa{38.003314116920116}
\def\wallthicknessapstagetwoa{10.76100316923541}
\def\collagenmassfractionapstagetwoa{0.099990853076329}
\def\timepointbpstagetwoa{900.5}
\def\pressurebpstagetwoa{140.0}
\def\myocytestressbpstagetwoa{22.320175704857355}
\def\diameterbpstagetwoa{57.81977156698272}
\def\wallthicknessbpstagetwoa{8.326654638067867}
\def\collagenmassfractionbpstagetwoa{0.16063522753367787}


==> supplementary_materials/figures/data/metrics_s140_1.tex <==
\def\myocytehomeostaticstresspstagetwob{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwob{10.761044144526878}
\def\cavitydiameterpstagetwob{37.99325395114782}
\def\timepointapstagetwob{0.0}
\def\pressureapstagetwob{120.0}
\def\myocytestressapstagetwob{22.02257643915123}
\def\diameterapstagetwob{37.990492240318716}
\def\wallthicknessapstagetwob{10.760539770234908}
\def\collagenmassfractionapstagetwob{0.1000022361719026}
\def\timepointbpstagetwob{1328.5}
\def\pressurebpstagetwob{140.0}
\def\myocytestressbpstagetwob{22.024182482227417}
\def\diameterbpstagetwob{45.47676555981399}
\def\wallthicknessbpstagetwob{9.501734110846582}
\def\collagenmassfractionbpstagetwob{0.12326161508607952}


==> supplementary_materials/figures/data/metrics_s140_243.tex <==
\def\myocytehomeostaticstresspstagetwog{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwog{10.761044144526878}
\def\cavitydiameterpstagetwog{37.97111782504683}
\def\timepointapstagetwog{0.0}
\def\pressureapstagetwog{120.0}
\def\myocytestressapstagetwog{22.02278315597887}
\def\diameterapstagetwog{37.97098472426861}
\def\wallthicknessapstagetwog{10.761048550539796}
\def\collagenmassfractionapstagetwog{0.10000354766853382}
\def\timepointbpstagetwog{229.0}
\def\pressurebpstagetwog{140.0}
\def\myocytestressbpstagetwog{22.022761704238413}
\def\diameterbpstagetwog{38.4309170788811}
\def\wallthicknessbpstagetwog{10.562026691903824}
\def\collagenmassfractionbpstagetwog{0.10065572067861417}


==> supplementary_materials/figures/data/metrics_s140_27.tex <==
\def\myocytehomeostaticstresspstagetwoe{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoe{10.761044144526878}
\def\cavitydiameterpstagetwoe{37.98754296280138}
\def\timepointapstagetwoe{0.0}
\def\pressureapstagetwoe{120.0}
\def\myocytestressapstagetwoe{22.022684177941386}
\def\diameterapstagetwoe{37.975881882052676}
\def\wallthicknessapstagetwoe{10.76075600740356}
\def\collagenmassfractionapstagetwoe{0.10000796488464152}
\def\timepointbpstagetwoe{301.0}
\def\pressurebpstagetwoe{140.0}
\def\myocytestressbpstagetwoe{22.022846322413084}
\def\diameterbpstagetwoe{39.129839946273506}
\def\wallthicknessbpstagetwoe{10.442232848072882}
\def\collagenmassfractionbpstagetwoe{0.10275356694947045}


==> supplementary_materials/figures/data/metrics_s140_3.tex <==
\def\myocytehomeostaticstresspstagetwoc{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoc{10.761044144526878}
\def\cavitydiameterpstagetwoc{37.973852415698175}
\def\timepointapstagetwoc{0.0}
\def\pressureapstagetwoc{120.0}
\def\myocytestressapstagetwoc{22.022758872012716}
\def\diameterapstagetwoc{37.988453536134145}
\def\wallthicknessapstagetwoc{10.760344155571936}
\def\collagenmassfractionapstagetwoc{0.10000947010343447}
\def\timepointbpstagetwoc{677.5}
\def\pressurebpstagetwoc{140.0}
\def\myocytestressbpstagetwoc{22.023592759552812}
\def\diameterbpstagetwoc{41.952050164040166}
\def\wallthicknessbpstagetwoc{9.98097168828223}
\def\collagenmassfractionbpstagetwoc{0.1120256682317859}


==> supplementary_materials/figures/data/metrics_s140_81.tex <==
\def\myocytehomeostaticstresspstagetwof{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwof{10.761044144526878}
\def\cavitydiameterpstagetwof{37.973171234540985}
\def\timepointapstagetwof{0.0}
\def\pressureapstagetwof{120.0}
\def\myocytestressapstagetwof{22.0227338109269}
\def\diameterapstagetwof{37.9659369685692}
\def\wallthicknessapstagetwof{10.760952666167386}
\def\collagenmassfractionapstagetwof{0.1000049472779319}
\def\timepointbpstagetwof{254.0}
\def\pressurebpstagetwof{140.0}
\def\myocytestressbpstagetwof{22.02277715212201}
\def\diameterbpstagetwof{38.64680992459487}
\def\wallthicknessbpstagetwof{10.527283352052004}
\def\collagenmassfractionbpstagetwof{0.10123420951367926}


==> supplementary_materials/figures/data/metrics_s140_9.tex <==
\def\myocytehomeostaticstresspstagetwod{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwod{10.761044144526878}
\def\cavitydiameterpstagetwod{37.97771347274108}
\def\timepointapstagetwod{0.0}
\def\pressureapstagetwod{120.0}
\def\myocytestressapstagetwod{22.022716368868238}
\def\diameterapstagetwod{37.975187375950405}
\def\wallthicknessapstagetwod{10.760440284747107}
\def\collagenmassfractionapstagetwod{0.10001182107091391}
\def\timepointbpstagetwod{424.5}
\def\pressurebpstagetwod{140.0}
\def\myocytestressbpstagetwod{22.023119725211615}
\def\diameterbpstagetwod{40.1632035746836}
\def\wallthicknessbpstagetwod{10.267605623789398}
\def\collagenmassfractionbpstagetwod{0.1060979560883707}


==> supplementary_materials/figures/data/metrics_s180_0.33.tex <==
\def\myocytehomeostaticstresspstagetwoa{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoa{10.761044144526878}
\def\cavitydiameterpstagetwoa{37.97807748655915}
\def\timepointapstagetwoa{0.0}
\def\pressureapstagetwoa{120.0}
\def\myocytestressapstagetwoa{22.021899769774404}
\def\diameterapstagetwoa{38.003314116920116}
\def\wallthicknessapstagetwoa{10.76100316923541}
\def\collagenmassfractionapstagetwoa{0.099990853076329}
\def\timepointbpstagetwoa{50.0}
\def\pressurebpstagetwoa{180.0}
\def\myocytestressbpstagetwoa{23.802518022443518}
\def\diameterbpstagetwoa{44.450459628454624}
\def\wallthicknessbpstagetwoa{9.803945208699716}
\def\collagenmassfractionbpstagetwoa{0.1206160142349238}


==> supplementary_materials/figures/data/metrics_s180_1.tex <==
\def\myocytehomeostaticstresspstagetwob{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwob{10.761044144526878}
\def\cavitydiameterpstagetwob{37.99325395114782}
\def\timepointapstagetwob{0.0}
\def\pressureapstagetwob{120.0}
\def\myocytestressapstagetwob{22.02257643915123}
\def\diameterapstagetwob{37.990492240318716}
\def\wallthicknessapstagetwob{10.760539770234908}
\def\collagenmassfractionapstagetwob{0.1000022361719026}
\def\timepointbpstagetwob{431.0}
\def\pressurebpstagetwob{180.0}
\def\myocytestressbpstagetwob{23.080600460769777}
\def\diameterbpstagetwob{68.19942571701}
\def\wallthicknessbpstagetwob{7.446502891513393}
\def\collagenmassfractionbpstagetwob{0.2540101805038529}


==> supplementary_materials/figures/data/metrics_s180_243.tex <==
\def\myocytehomeostaticstresspstagetwog{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwog{10.761044144526878}
\def\cavitydiameterpstagetwog{37.97111782504683}
\def\timepointapstagetwog{0.0}
\def\pressureapstagetwog{120.0}
\def\myocytestressapstagetwog{22.02278315597887}
\def\diameterapstagetwog{37.97098472426861}
\def\wallthicknessapstagetwog{10.761048550539796}
\def\collagenmassfractionapstagetwog{0.10000354766853382}
\def\timepointbpstagetwog{312.0}
\def\pressurebpstagetwog{180.0}
\def\myocytestressbpstagetwog{22.022875387044365}
\def\diameterbpstagetwog{39.34842014051796}
\def\wallthicknessbpstagetwog{10.179385371334574}
\def\collagenmassfractionbpstagetwog{0.10215618625965507}


==> supplementary_materials/figures/data/metrics_s180_27.tex <==
\def\myocytehomeostaticstresspstagetwoe{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoe{10.761044144526878}
\def\cavitydiameterpstagetwoe{37.98754296280138}
\def\timepointapstagetwoe{0.0}
\def\pressureapstagetwoe{120.0}
\def\myocytestressapstagetwoe{22.022684177941386}
\def\diameterapstagetwoe{37.975881882052676}
\def\wallthicknessapstagetwoe{10.76075600740356}
\def\collagenmassfractionapstagetwoe{0.10000796488464152}
\def\timepointbpstagetwoe{406.5}
\def\pressurebpstagetwoe{180.0}
\def\myocytestressbpstagetwoe{22.02293782974717}
\def\diameterbpstagetwoe{41.602204405454316}
\def\wallthicknessbpstagetwoe{9.843481427441295}
\def\collagenmassfractionbpstagetwoe{0.11028213619192251}


==> supplementary_materials/figures/data/metrics_s180_3.tex <==
\def\myocytehomeostaticstresspstagetwoc{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwoc{10.761044144526878}
\def\cavitydiameterpstagetwoc{37.973852415698175}
\def\timepointapstagetwoc{0.0}
\def\pressureapstagetwoc{120.0}
\def\myocytestressapstagetwoc{22.022758872012716}
\def\diameterapstagetwoc{37.988453536134145}
\def\wallthicknessapstagetwoc{10.760344155571936}
\def\collagenmassfractionapstagetwoc{0.10000947010343447}
\def\timepointbpstagetwoc{708.5}
\def\pressurebpstagetwoc{180.0}
\def\myocytestressbpstagetwoc{22.38562335878783}
\def\diameterbpstagetwoc{64.00730348764574}
\def\wallthicknessbpstagetwoc{7.233926890397889}
\def\collagenmassfractionbpstagetwoc{0.20972144311307386}


==> supplementary_materials/figures/data/metrics_s180_81.tex <==
\def\myocytehomeostaticstresspstagetwof{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwof{10.761044144526878}
\def\cavitydiameterpstagetwof{37.973171234540985}
\def\timepointapstagetwof{0.0}
\def\pressureapstagetwof{120.0}
\def\myocytestressapstagetwof{22.0227338109269}
\def\diameterapstagetwof{37.9659369685692}
\def\wallthicknessapstagetwof{10.760952666167386}
\def\collagenmassfractionapstagetwof{0.1000049472779319}
\def\timepointbpstagetwof{331.0}
\def\pressurebpstagetwof{180.0}
\def\myocytestressbpstagetwof{22.022886994010456}
\def\diameterbpstagetwof{39.99044759552984}
\def\wallthicknessbpstagetwof{10.085092917227717}
\def\collagenmassfractionbpstagetwof{0.10421860464531123}


==> supplementary_materials/figures/data/metrics_s180_9.tex <==
\def\myocytehomeostaticstresspstagetwod{22.02277748047476}
\def\midcavityrefwallthicknesspstagetwod{10.761044144526878}
\def\cavitydiameterpstagetwod{37.97771347274108}
\def\timepointapstagetwod{0.0}
\def\pressureapstagetwod{120.0}
\def\myocytestressapstagetwod{22.022716368868238}
\def\diameterapstagetwod{37.975187375950405}
\def\wallthicknessapstagetwod{10.760440284747107}
\def\collagenmassfractionapstagetwod{0.10001182107091391}
\def\timepointbpstagetwod{756.0}
\def\pressurebpstagetwod{180.0}
\def\myocytestressbpstagetwod{22.02326579967937}
\def\diameterbpstagetwod{45.99104445918943}
\def\wallthicknessbpstagetwod{9.220541197362996}
\def\collagenmassfractionbpstagetwod{0.12785873909585707}

